QChecker: Detecting Bugs in Quantum Programs via Static Analysis

Static analysis is the process of analyzing software code without executing the software. It can help find bugs and potential problems in software that may only appear at runtime. Although many static analysis tools have been developed for classical software, due to the nature of quantum programs, these existing tools are unsuitable for analyzing quantum programs. This paper presents QChecker, a static analysis tool that supports finding bugs in quantum programs in Qiskit. QChecker consists of two main modules: a module for extracting program information based on abstract syntax tree (AST), and a module for detecting bugs based on patterns. We evaluate the performance of QChecker using the Bugs4Q benchmark. The evaluation results show that QChecker can effectively detect various bugs in quantum programs.

==> sections/back.tex <==
\section{Background}\label{sec:background}


We briefly introduce the background information on programming in Qiskit and the basic concepts of qubits.

\subsection{Qiskit}

Qiskit~\cite{aleksandrowicz2019qiskit} is one of the most widely used open-source frameworks for quantum computing, allowing us to create algorithms for quantum computers. As a Python package, it provides tools for creating and manipulating quantum programs and running on prototype quantum devices and simulators and can use built-in modules for noise characterization and circuit optimization to reduce the impact of noise. Qiskit also provides a library of quantum algorithms for machine learning, optimization, and chemistry.
%Qiskit provides a complete set of tools needed to interact with quantum systems and simulators and 

In Qiskit, a program is defined by a quantum object data structure that contains configuration information and the experiment sequences. The object can be used to get status information and retrieve results~\cite{mckay2018qiskit}.
Figure~\ref{fig:mesh1} shows a simple Qiskit program that illustrates the entire workflow of a quantum program. 
%In Qiskit, we need first to create a backend simulator \CodeIn{qasm\_simulator} as follows.
The function \CodeIn{Aer.get\_backend('qasm\_simulator')} returns a backend object for the given backend name (\CodeIn{qasm\_simulator}). 
The \CodeIn{backend} class is an interface to the simulator, and the actual name  of \CodeIn{Aer} for this class is \CodeIn{AerProvider}.
\noindent
After the experimental design is completed, the instructions are run through the \CodeIn{execute} method.
The \CodeIn{shots} of the simulation, which means the number of times the circuit is run, is set to 1000 while the default is 1024.
When outputting the results of a measurement, the method \CodeIn{job.result()} is used to retrieve the measurement results. We can access the counts via the method \CodeIn{get\_counts(circuit)}, which gives the experiment's aggregate outcomes.

%IBM offers an online platform, "IBM Quantum Experience~\cite{IBM}," which features two 5-qubit processors and one 16-qubit processor, making it very powerful. We can use Qiskit to build the circuit directly in the online backend. It is also possible to program locally using Qiskit in a standalone Jupyter programming environment. Another powerful aspect of Qiskit is that there is no need to do the manual work of unassigning qubits, making programming with Qiskit becomes much easier and more efficient.

\subsection{Basic Properties of Qubits}
In the following, we use Qiskit as an example to explain the characteristics of quantum bit (qubit for short) and the necessary execution process of a complete quantum program.

\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}
    simulator = \textbf{Aer.get_backend}("qasm_simulator")

    qreg = \textbf{QuantumRegister}(3)
    creg = \textbf{ClassicalRegister}(3)
    circuit = \textbf{QuantumCircuit}(qreg, creg)

    circuit.\textbf{h}(0)
    circuit.\textbf{h}(2)
    circuit.\textbf{cx}(0, 1)
    circuit.\textbf{measure}([0,1,2], [0,1,2])
    job = \textbf{execute}(circuit, simulator, shots=1000)
    result = job.\textbf{result}()
    counts = result.\textbf{get_counts}(circuit)
    \textbf{print}(counts)
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:mesh1}A simple quantum program in Qiskit}
\end{figure}

The basic unit of information in quantum computing is the qubit. As shown in Figure~\ref{fig:mesh1}, \CodeIn{qreg = QuantumRegister(3)} means assigning a quantum register of three qubits, and the value of each qubit is $\ket{0}$ by default. So the initial value of these three qubits is $\ket{000}$. Next, let the first and third qubits pass through the H (Hadamard) gate, as shown by \CodeIn{circuit.h(0)} and \CodeIn{circuit.h(2)}. In this way, the unique property {\it superposition} of qubits is realized, which means the qubit contains the states of $\ket{0}$ and $\ket{1}$.
There is also an {\it entanglement} of qubit properties that only multiple qubits can achieve. The code in the sample program is \CodeIn{circuit.cx(0,1)}. That is to say, the first qubit is entangled with the second qubit through a CNOT (Controlled-NOT) gate operation. We measure the first qubit, and its output is \CodeIn{0} for 50 percent probability and \CodeIn{1} for 50 percent probability. After that, measuring the second qubit is 100 percent the same as the first measurement result.
Since the third qubit is not related to the first two qubits, the last qubit's measurement result is still taken with \CodeIn{0} for 50 percent probability and \CodeIn{1} for 50 percent probability.
The measurement statement of qubits shown in Figure~\ref{fig:mesh1} is \CodeIn{circuit.measure([0,1,2], [0,1,2])}. Measurement can lead to the collapse of a quantum superposition state to a classical state. There are many kinds of quantum measurements, and the projection measurement of a single qubit is used here. That is, each qubit is projected onto a state space consisting of base vectors $\ket{0}$ or $\ket{1}$. In this program, the final output is a three-bit array.





\iffalse
%\zpz{In this section, we briefly introduce some basic concepts of quantum computing, followed by an introduction to Qiskit and quantum programming features with an example program.}
In this section, we briefly introduce Qiskit with a simple example, followed by some basic concepts to better understand quantum programming. Finally, is our conclusion of quantum program features.



\subsection{Qiskit}
\label{subsec:qiskit}

Several open-source programming frameworks, such as Qiskit~\cite{ibm2021qiskit}, Q\#~\cite{svore2018q}, Scaffold~\cite{abhari2012scaffold} and ProjectQ~\cite{haner2016high}, have been proposed for supporting quantum programming recently, which are used further to advance the implementation and application of quantum algorithms. We can use these frameworks to develop quantum programs. This paper chooses Qiskit, one of the most widely used quantum programming languages, as the first target language for conducting our work.

Qiskit is one of the most widely used open-source frameworks for quantum computing, allowing us to create algorithms for quantum computers~\cite{koch2019introduction}. As a Python package, it provides tools to create and manipulate quantum programs running on prototype quantum devices and simulators~\cite{aleksandrowicz2019qiskit}. In addition, It can use built-in modules for noise characterization and circuit optimization to reduce the impact of noise. It also provides a library of quantum algorithms for machine learning, optimization, and chemistry.
%Qiskit provides a complete set of tools needed to interact with quantum systems and simulators and 
In Qiskit, an experiment is defined by a quantum object data structure that contains configuration information and the experiment sequences. The object can be used to get status information and retrieve results~\cite{mckay2018qiskit}. Figure~\ref{fig:mesh1} shows a simple Qiskit program that illustrates the entire workflow of a quantum program. 
%In Qiskit, we need to create a backend simulator \CodeIn{qasm\_simulator} as follows.
The function \CodeIn{Aer.get\_backend('qasm\_simulator')} returns a backend object for the given backend name (\CodeIn{qasm\_simulator}). The \CodeIn{backend} class is an interface to the simulator, and the actual name  of \CodeIn{Aer} for this class is \CodeIn{AerProvider}.
\noindent
After the experimental design is completed, the instructions are run through the \CodeIn{execute} method. The \CodeIn{shots} of the simulation, which means that the number of times the circuit is run, is set to 1000 while the default is 1024. When outputting the results of a measurement, the method \CodeIn{job.result()} is used to retrieve the measurement results. We can access the counts via the method \CodeIn{get\_counts(circuit)}, which gives the experiment's aggregate outcomes.

\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}
    simulator = \textbf{Aer.get_backend}('qasm_simulator')

    qreg = \textbf{QuantumRegister}(3)
    creg = \textbf{ClassicalRegister}(3)
    circuit = \textbf{QuantumCircuit}(qreg, creg)

    circuit.\textbf{h}(0)
    circuit.\textbf{h}(2)
    circuit.\textbf{cx}(0, 1)
    circuit.\textbf{measure}([0,1,2], [0,1,2])
    job = \textbf{execute}(circuit, simulator, shots=1000)
    result = job.\textbf{result}()
    counts = result.\textbf{get_counts}(circuit)
    \textbf{print}(counts)
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:mesh1} A sample quantum program in Qiskit.}
\end{figure}


\iffalse
Figure~\ref{fig:mesh1} is an example of Qiskit programs\footnote{\url{https://github.com/Qiskit/qiskit-terra/blob/main/examples/Python/ibmq/hello_quantum.py}}.
\fi

\subsection{Basic Concepts}

A quantum bit (qubit) is the analog of one classical bit but has many different properties. A classical bit, like a coin, has only two states, 0 and 1, while a qubit can be in a continuum of states between $\Ket{0}$ and $\Ket{1}$ in which the $\Ket{}$ notation is called Dirac notation. We can represent a qubit mathematically as $\Ket{\psi} = \alpha\Ket{0} + \beta\Ket{1}$ where $|\alpha|^2 + |\beta|^2 = 1$ and the numbers $\alpha$ and $\beta$ are complex numbers. The states $\Ket{0}$ and $\Ket{1}$ are called computational basis states. Unlike classical bits, we cannot examine a qubit directly to get the values of $\alpha$ and $\beta$. Instead, we measure a qubit to obtain either the result 0 with probability $|\alpha|^2$ or the result 1 with probability $|\beta|^2$.

Quantum gates are used for quantum computation and manipulating quantum information. Some basic quantum gates are as follows:
\begin{itemize}[leftmargin=2em]
\setlength{\itemsep}{3pt}
  \item Quantum NOT gate takes the state $\Ket{\psi} = \alpha\Ket{0} + \beta\Ket{1}$ into the state $\Ket{\psi} = \alpha\Ket{1} + \beta\Ket{0}$. We can use a matrix to represent this operation:
  \begin{gather*}X = \begin{bmatrix} 0 & 1\\1 & 0\end{bmatrix}\end{gather*}
  \item The Z gate can be expressed as 
  \begin{gather*}Z = \begin{bmatrix} 1 & 0 \\ 0 & -1\end{bmatrix}\end{gather*} 
  From the matrix, we know the Z gate leaves the $\Ket{0}$ unchanged and changes the sign of $\Ket{1}$.
  \item The Hadamard gate turns the $\Ket{0}$ into $(\Ket{0} + \Ket{1})/\sqrt{2}$ and turns the $\Ket{1}$ into $(\Ket{0} - \Ket{1})/\sqrt{2}$. The matrix form of the Hadamard gate is 
  \begin{gather*}H = \frac{1}{\sqrt{2}}\begin{bmatrix} 1 & 1\\ 1 & -1 \end{bmatrix}\end{gather*}
\end{itemize}

All the matrices are unitary ones. Besides these single-qubit gates, there are multiple qubit gates, such as the Controlled-NOT gate (CNOT gate). This gate has two input qubits, the control qubit, and the target qubit. If the control qubit is 0, then the target qubit remains unchanged. If the control qubit is 1, then the target qubit is flipped. We can express the behavior of the CNOT gate as $\Ket{A, B} \rightarrow \Ket{A, B \oplus A}$. 
\iffalse
The matrix representation is 
\begin{gather*}U_{CN} = \begin{bmatrix}  1 & 0 & 0 & 0 \\ 0 & 1 & 0 & 0 \\ 0 & 0 & 0 & 1 \\ 0 & 0 & 1 & 0 \end{bmatrix}\end{gather*}
\fi

Quantum circuits are models of all kinds of quantum processes. We can build quantum circuits with quantum gates and use wires to connect the components in quantum circuits. These wires can represent the passage of time or a physical particle moving from one position to another. Another essential operation in quantum circuits is measurement. Measurement operation observes a single qubit and obtains a classic bit with a certain probability. Nielsen's book~\cite{nielsen2002quantum} has a more detailed explanation of quantum computation.

\subsection{Quantum Program Features}
\label{subsec:program features}
A quantum program is a series of operations on qubits.
By focusing on the quantum program language features, we can
classify a complete quantum program into the following four
steps:

\begin{itemize}[leftmargin=2em]\setlength{\itemsep}{3pt}
  \item {\bf Initialization}: The initial stage is to initialize the quantum registers to store the qubits that need to be manipulated. Then the classical registers are initialized to store the values of the measured qubits.
  As shown in Figure~\ref{fig:mesh1}, \CodeIn{qreg = QuantumRegister(3)} means assigning a quantum register of three qubits, and the value of each qubit is $\ket{0}$ by default. So the initial value of these three qubits is $\ket{000}$.
  
  \item {\bf Gate Operation}: The core of quantum computing is to operate on qubits. Qiskit provides almost all the gates to implement algorithms in quantum programs~\cite{IBM}.
  Such as, to achieve the superposition of qubits, it must pass through the H (Hadamard) Gate (e.g., \CodeIn{circuit.h(0)} \& \CodeIn{circuit.h(2)}). 
  And To achieve "entanglement" in the case of multiple qubits, it must pass through the CNOT ( controlled-NOT) gate (e.g., \CodeIn{circuit.cx(0,1)}). Complex gate operations are decomposed into basic gates in quantum language and gradually realized. Two qubits parameterize controlled gates, and double-controlled gates require three qubits. 
 
  \item {\bf Measurement}: When we want to obtain the output, we must perform a measurement operation on the target qubit. The measured qubit is returned as the classical state's value, which no longer has superposition properties. So the qubit that has been measured cannot be used as a control qubit to entangle with other qubits. Although measurement is a simple operation, the program executing a measurement statement is very complicated. It requires thousands of projection measurements of the qubits to output the counts. In this way, the number of occurrences of the result is used to obtain the size of the probability of outputting the value. The measurement statement of qubits shown in Figure~\ref{fig:mesh1} is \CodeIn{circuit.measure([0,1,2], [0,1,2])}.
  
  \item {\bf Deallocation}: It is critical to reset and release qubits safely; otherwise, ancilla qubits in an entangled state will affect the output, i.e., by the measurement of the target qubit. For some backends of Qiskit or other quantum programming languages, failure to reset the temporary value to zero and release it safely may lead to program bugs.
  
    %Deallocation is not considered a specific operation due to the power of Qiskit. We do not need to reset the qubits manually. 

The four aspects are the main part of the quantum program. 
\end{itemize}
\fi



==> sections/conclusion.tex <==
\section{Conclusion Remarks}\label{sec:conclusion}

%Existing static analysis tools fail to detect the potential bugs of quantum programs since quantum programs have significantly different properties from traditional programs. 

In this paper, we have presented QChecker, a static analysis tool for quantum programs to enable effective and efficient potential bug detection of quantum programs. QChecker involves two AST-based program information extraction modules and comprehensive bug detectors which can detect various bug patterns. We applied QChecker to the Bugs4Q benchmark suite and evaluated its effectiveness. The results show that QChecker can detect various types of bugs in quantum programs. 
%
In the future, we plan to extend QChecker for detecting more bug patterns of Qiskit programs and supporting bug detection of other common quantum programming languages such as Cirq and ProjectQ.

%In the future, we plan to extend QChecker for more functionality, e.g., automatic test case generation, impact analysis, and metrics analysis. We will also incorporate more quantum simulation modules with bug detection. With the increasing number of quantum programming bugs, new bug types will be involved in QChecker, simultaneously. Moreover, QChecker will also be extended to detect program bugs in other common quantum programming languages.


==> sections/experiment.tex <==

\section{Evaluation}
% 缺少检测时间的实验；以及precision，recall和F1的计算
%add environment:python3.10...
\label{sec:experiments}
This section presents the empirical performance of QChecker. We evaluate QChecker on Bugs4Q~\cite{zhao2021bugs4q}, which contains 42 real-world buggy quantum programs in Qiskit. The experiments were conducted on a server with an Intel i9-10940X CPU, 128G RAM, running on Ubuntu 20.04 with Python 3.10 installed.

% All the experiments are conducted on a server with CPU (Intel(R) Core(TM) i9-10940X CPU @ 3.30GHz), 128GB RAM, and Python version of 3.10. 
%Interestingly, we found that QChecker is very slight and requires minimal computation resources. Moreover, QChecker supports the main-stream operating systems such as MS-Windows, Linux, and MacOS.

\subsection{Metrics}
We adopt \emph{Precision}, \emph{Recall}, and \emph{F1-score} to evaluate the performance of QChecker. Specifically, for each bug \emph{b} in Bugs4Q, we use the bug type in Bugs4Q as ground-truth and apply QChecker to its source quantum program. If the detection result of QChecker matches the corresponding bug type in Bugs4Q, we call this \emph{b} as \emph{True Positive} (TP). Otherwise, this \emph{b} is a \emph{False Positive} (FP). \emph{False Negative} (FN) is a ground-truth bug that can not be detected by QChecker. The \emph{Precision} is calculated as 
\begin{math}TP/ (TP + FP)\end{math}, \emph{Recall} as \begin{math}TP/(TP + FN)\end{math} and \emph{F1-score} as \begin{math}
2 \times Precision \times Recall / (Precision + Recall)
\end{math}. 
\subsection{Performance on Real-World Qiskit Programs}
First of all, there are 42 Qiskit programs detected by QChecker, and 24 bugs were found. 
Figure~\ref{fig:9} shows the empirical results produced by applying QChecker on Bugs4Q. 
Detector \CodeIn{PE} found 10 bugs, while \CodeIn{CE} and \CodeIn{IS} found 7 and 2 bugs, respectively. And other detectors found one bug in each. As we know, out of the 42 bugs in Bugs4Q, 22 bugs are output errors, i.e., the output of the program does not match the user's expectations. This condition makes Qchercker unable to detect these bugs. So we consider that the remaining number of bugs in Bugs4Q found by Qchecker is in line with expectations.
Combining Table~\ref{table:1} with the results in Figure~\ref{fig:9}, we analyzed and derived two points about the performance of each detector:
\begin{itemize}[leftmargin=2em]
\setlength{\itemsep}{3pt}

   \item \textit{The more cases the detectors can cover, the more bugs can be found}. As we made the detectors according to the relevance of the bug patterns, the number of cases covered by each detector may vary. Detector \CodeIn{PE} and \CodeIn{CE} can detect more cases than other detectors. And in fact, the two detectors made a better performance. 

   \item \textit{The performance of detectors also depends on the type of errors made by the programmers}. 
   Considering the limited number of bugs in Bugs4Q, we believe that some detectors perform poorly because they cover cases that rarely occur. For example, detector \CodeIn{IG}, \CodeIn{CM}, and \CodeIn{IS} can detect more than one case while the results are barely satisfactory. 
   %Therefore, we believe that most of the bugs come from parameter errors and call errors.
 \end{itemize}


 In addition, a detector that solves only one case does not indicate poor performance.
 Instead, with their increased functionality, these specialized detectors will realize their potential to detect bugs better.

\begin{figure}[h]
    \centering
    \includegraphics[width=0.45\textwidth]{222.png}
    \caption{Distribution of bugs found by each detector.}
    \label{fig:9}

\end{figure}
\begin{table}
\centering
\caption{Performance of QChecker on Qiskit programs.}

\label{tbl:qc_performance}
\begin{tabular}{l|cccc}
\toprule
Performance & \emph{Prec.} & \emph{Recall} & \emph{F1-score} & \emph{Avg. Time}\\
\midrule
QChecker & 0.625 & 0.882 & 0.731 & 48.2ms \\
\bottomrule
\end{tabular}
\end{table}

The performance of QChecker on Qiskit programs is also
shown in Table~\ref{tbl:qc_performance}. 
% Compared to static analysis tools for traditional programs~\cite{li2019vbsac}, QChecker has achieved reasonable performance in detecting bugs in quantum programs. 
As illustrated in \cite{matteo2022morphq}, executing a quantum program on simulators can easily consume more than \begin{math}10^3\end{math} ms. QChecker only takes 48.2 ms for full detection on a single quantum program, exhibiting the efficiency of QChecker.

\subsection{Extendability of QChecker}
% Although QChecker was developed for Qiskit programs, we tried to apply QChecker to other Python-based quantum programming languages.
%{\color{red}{Although QChecker is targeted at quantum programs written in Qiskit, we try to apply QChecker to seven buggy Cirq programs to evaluate its performance on other Python-based quantum languages. The results show that only one out of the seven bugs is detected by QChecker.}}
%Bugs4Q contains seven buggy programs written in Cirq. 
The example of a Cirq program and the corresponding detection result of QChecker are shown in Figures~\ref{fig:10} and \ref{fig:11}, respectively. After careful inspection of the results, we find that the information extraction part of QChecker can still function on other Python-based quantum languages (e.g., Cirq). The syntax difference between these quantum languages will cause the detectors designed for Qiskit fails to work, which may lead to the lack of guaranteed performance.
%We can see almost information is extracted by QChecker so that the detectors can function.
%Between the seven buggy programs provided in Bugs4Q, one bug was found by the detector \CodeIn{IG}.
% From the evaluation, we consider QChecker can be used for common Python-based quantum programming languages.

\begin{tcolorbox}[size=title]
{The experimental results show that QChecker can successfully detect bugs in real-world Qiskit quantum programs, exhibiting the effectiveness of applying static analysis to quantum programs. %Although QChecker suffers significant performance degradation on Cirq programs, 
Besides, the intermediate results indicate that the QChecker can correctly extract the \CodeIn{QP\_Attribute} and \CodeIn{QP\_Operation} information from the underlying Cirq program, indicating that the QChecker can be easily extended to common Python-based quantum programming languages.
}
\end{tcolorbox}
\begin{figure}[t]
\begin{CodeOut}
    \footnotesize{
  \begin{alltt}
    \textbf{import} cirq
    qubit = cirq.\textbf{NamedQubit}("myqubit")
    circuit = cirq.\textbf{Circuit}(cirq.H(qubit))
    \textbf{for} i \textbf{in} range(10):
        result2 = cirq.\textbf{measure}(qubit, key='myqubit')
        \textbf{print}(result2)
    \textbf{print}(circuit)
    result = cirq.\textbf{Simulator()}.simulate(circuit)
    \textbf{print}(result2)
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:10}An exapmle of Cirq program.}
\end{figure}

\begin{figure}[t]
\begin{CodeOut}
    \footnotesize{
    \begin{alltt}
    ('qubit', 'cirq.\textbf{NamedQubit}("myqubit")')
    ('circuit', 'cirq.\textbf{Circuit}(cirq.H(qubit))') 
    ('result', 'cirq.\textbf{Simulator}().simulate(circuit)')
    ('result2', 'cirq.\textbf{measure}(qubit,key="myqubit")')
    ==========================================
    'cirq.\textbf{NamedQubit}("myqubit")'
    'cirq.\textbf{Circuit}(cirq.H(qubit))'
    'range(10)'
    '\textbf{print}(circuit)'
    'cirq.\textbf{Simulator()}.simulate(circuit)'
    '\textbf{print}("result:")'
    '\textbf{print}(result2)'
    'cirq.\textbf{H}(qubit)'
    'cirq.\textbf{measure}(qubit,key="myqubit")',
    '\textbf{print}(result2)',
    'cirq.\textbf{Simulator()}'
\end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:11}A Cirq program detected by QChecker}
\end{figure}





==> sections/intro.tex <==
\section{Introduction}
Recent advances in hardware have inspired the innovation of quantum software engineering~\cite{zhao2020quantum,piattini2020quantum} from both industry and academia. Due to its unique promising advantage over classical computing, quantum computing has been applied to many cutting-edge areas, e.g., quantum machine learning~\cite{biamonte2017quantum, dunjko2016quantum}, big data analysis~\cite{rebentrost2014quantum}, and molecular simulations~\cite{grimsley2019adaptive}. 
Quantum programming is designing and constructing executable quantum programs to achieve a specific computational result.
With the rapidly growing complexity of quantum programs, it is decisive to alleviate the efforts in programming such quantum programs. 
%\textcolor{blue}{Quantum computing frameworks are for this rapidly emerging field of what deep learning (DL) frameworks and execution environments are for DL programs.} 
Several quantum programming languages are available for quantum programmers, such as Qiskit~\cite{aleksandrowicz2019qiskit}, Q\#~\cite{svore2018q}, Quipper~\cite{green2013quipper}, and Cirq~\cite{cirq2018google}, allowing researchers and developers to implement and experiment with various quantum computing techniques quickly. 

Given the importance and wide application of quantum programming, ensuring the correctness of quantum programs is crucial for quantum software development. However, recent empirical studies~\cite{zhao2021bugs4q, zhao2021identifying,paltenghi2021bugs, campos2021qbugs} have shown that the current quantum program development process is still error-prone. While testing quantum programs has gained significant attention~\cite{wang2021quito, gely2020qucat,wang2021generating, mendiluze2021muskit,long2022testing, fortunato2022mutation}, the existing testing techniques (e.g., mutation testing, metamorphic testing) often require dynamic execution of the underlying quantum programs. Considering that most of the current quantum programs are executed on quantum computers and simulators available on the cloud, the existing testing techniques can be slightly cumbersome and expensive.

%Static analysis tools are programs that aim at inferring program properties of other programs by examining the source of other programs without running them. 
Static analysis for traditional programs has been extensively studied and has been widely adopted in modern development practices~\cite{radhika2014static, wang2022icpc}. 
Due to the advantage in speed and cost, static bug finders (also known as static analyzers) that can infer program properties without program execution have been extensively studied and widely adopted in modern development practices to find bugs in traditional programs~\cite{venkatasubramanyam2014dynamic,hovemeyer2004finding}. However, detecting bugs in quantum programs via static analysis can be challenging. Since quantum computation logic is expressed in quantum circuits, and the states of quantum registers are measured probabilistically, static analysis tools designed for traditional programs struggle to detect mistakes in quantum programs. 

To bridge the gap, we present QChecker, the first static analysis tool designed for detecting bugs in quantum programs. The approach addresses the challenge above by first distilling a set of common bug patterns summarized from real quantum bugs in previous studies~\cite{zhao2021bugs4q,zhao2021identifying} and then using these bug patterns to construct eight detectors for quantum programs. The whole process is non-trivial since the distilled bug patterns must carefully consider the domain-specific constraints of quantum computing to be accurate and effective.

We evaluate QChecker on Bugs4Q~\cite{zhao2021bugs4q}, a realistic benchmark consisting of 42 real-world buggy quantum programs. 
%\textcolor{red}{Furthermore, we evaluate QChecker on seven buggy quantum programs written in Cirq.} 
Experimental results show that QChecker can efficiently detect bugs in quantum programs and \textcolor{red}{exhibit extendibility to common Python-based quantum programming languages. Furthermore, we discuss the extendability of QChercker for other python-based quantum programming languages.}

In summary, this work makes the following contributions:
\begin{itemize}[leftmargin=2em]
\setlength{\itemsep}{3pt}
\item We present the first bug detection tool dedicated to quantum programs in Qiskit. Using static analysis techniques, QChecker can generate diagnostic messages that assist developers in pinpointing potential bugs in their programs quickly.
\item We implement QChecker and evaluate its effectiveness and performance in a real-world Bugs4Q benchmark. The results show that QChecker can effectively detect various types of bugs in quantum programs. 
  % \item We distill a set of common bug patterns for quantum programs, which is the foundation of performing static analysis on quantum programs.
%  \item We propose a novel approach of decomposition that represents quantum programs using \CodeIn{QP\_Operation} and \CodeIn{QP\_Attribute}, which is the foundation of performing static analysis on quantum programs.
%  \item We construct eight detectors based on our proposed bug patterns to enable the first static analysis tool for quantum programs. 
%  \item We integrate QChecker with the widely used Qiskit framework and have tested its extendibility to other Python-based quantum programming languages.
  
  % \item It avoids the collapse of quantum states caused by prying into the internal quantum state.
  
  % \item It saves the time and resources needed to test quantum programs dynamically.
  
  % \item It has proven effective in finding detects and vulnerabilities in Qiskit programs.
\end{itemize}

The rest of the paper is organized as follows. Section~\ref{sec:background} provides some basics of quantum programming. 
Section~\ref{sec:methodology} describes our QChecker approach for static analysis of quantum programs. Section~\ref{sec:experiments} presents the performance of QChecker on Bugs4Q. Section~\ref{sec:threats} reviews our threats of validity.
Section~\ref{sec:related} discusses related work, and Section~\ref{sec:conclusion} finally concludes this paper.

==> sections/method.tex <==
\begin{figure*}[h]
    \centering
    \includegraphics[width=0.9\textwidth]{structure.png}
    \caption{The structure of QChecker.}
    \label{fig:sketch}
\end{figure*}

\section{The QChecker Tool} \label{sec:methodology}
% In this section, we briefly introduce the construction of QChecker. 
% \Zhuo{In this section, we introduce the construction of QChecker. }
% QChecker is developed based on the Python language. We use the \textit{ast} module provided by Python to extract information from the program. The \textit{sys} and \textit{os} modules are used to implement QCheckcer's interaction with the system environment and the quantum program files under test. As well as the basic \textit{re} module to implement regular expression matching operations.
% Clearly, QChecker can achieve detection without the environment for executing quantum programs.

% %The QChecker tool is open-sourced at:{\color{red}?}.
% Figure~\ref{fig:sketch} shows how the QChecker finds bugs.
% First, the information of a quantum program is extracted by the \CodeIn{Ast\_operator} and decomposed into two parts: program attributes and program operation. Next, extracted information will be passed through the detectors.
% Finally, if bugs are found, QChecker will catch the bugs and provide information about the program and the error codes provided by detectors. If there is no bug detected, QChecker will return false.

In this section, we introduce the construction of QChecker, which is developed based on Python. As illustrated in Figure~\ref{fig:sketch}, QChecker first performs a thorough information extraction of the quantum programs based on their ASTs. The corresponding operations are in the module \CodeIn{Ast\_Operator}. The information mainly includes the variable assign operations and function calls, which will be further stored in \CodeIn{QP\_Attribute} and \CodeIn{QP\_Operation}. Then QChecker transmits the extracted information to the bug detectors. The bug detectors can detect various bug patterns (e.g., IG, IS).
Finally, QChecker generates bug detection reports, including the buggy programs, line numbers, and bug descriptions.

\subsection{Information Extraction}
% When QChecker receives a quantum program under test, the first thing is converting the program into the form of an abstract syntax tree (AST). 
% Next, QChecker provides two functions for information extraction: \CodeIn{QP\_Attribute} and \CodeIn{QP\_operation}. 

The previous static analysis tools inspire us (e.g., PyLint~\cite{thenault2001pylint}) that using AST for program information extraction is effective and efficient. However, different from traditional static analysis tools, the \CodeIn{AST\_Operator} in QChecker has the ability to extract information specific to the semantics and the function of quantum programs. Taking the program shown in Figure~\ref{fig:mesh1} as an example, we apply a structured parsing to each quantum program file, i.e., generating the AST. We adopt two modules named \CodeIn{QP\_Attribute} and \CodeIn{QP\_Operation} to store the AST information of all the variables and function calls, respectively. In addition, QChecker also supports handling complex syntax and data structures such as dictionaries, lists, function definitions, loops, and conditional branches. The purpose of this design is that the structured AST-based information extraction can help QChecker trace the relationship between each variable and function call. For example, a variable may be modified multiple times, or its name may be changed when passed as an argument inside a function.
Nevertheless, we can still trace back the initial value of the variables in the program. We plot instances of \CodeIn{QP\_Attribute} and \CodeIn{QP\_Operation} in Figures~\ref{fig:attr} and \ref{fig:opt}, respectively. %The bug detectors can detect various bug patterns (e.g., IG, IS).


\begin{itemize}[leftmargin=2em]
\setlength{\itemsep}{3pt}
  \item \textbf{QP\_Attribute}: The AST structure of a variable includes its variable name, variable value (which can come from a constant, another variable, or the result of a function calculation), type, and location (line of code). As shown in Figure~\ref{fig:attr}, The \CodeIn{QP\_Attribute} module is designed in a key-value manner. The keys are variable names which can be the indices for the variable values. 
  \item \textbf{QP\_Operation}: The AST structure of a function call contains a list of its arguments, the type and value of each argument, its position, and other information. As shown in Figure~\ref{fig:opt}, The \CodeIn{QP\_Operation} module is a list that contains all the function calls in the quantum program file. In detail, each function call can be further divided into function call names, arguments, and values. This information is stored in a more comprehensive table from QChecker, which uses the function call strings in \CodeIn{QP\_Operation} as the index.
\end{itemize}

These two modules contain all the information of a quantum program and make it more straightforward for further bug detection.
Moreover, users can directly obtain the above information through QChecker based on the API we released. It is worth mentioning that those programs containing basic syntax errors (e.g., python indentation errors, unrecognized operators, undefined variables and functions, etc.) will not be processed by QChecker. Instead, they will be prompted as syntax errors and thus be excluded from the static checking.


\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}
    ('simulator', '\textbf{Aer.get_backend}("qasm_simulator")') 
    ('qreg', '\textbf{QuantumRegister}(3)') 
    ('creg', '\textbf{ClassicalRegister}(3)') 
    ('circuit', '\textbf{QuantumCircuit}(qreg,creg)') 
    ('job', '\textbf{execute}(circuit,simulator,shots=1000)') 
    ('result', 'job.\textbf{result}()') 
    ('counts', 'result.\textbf{get_counts}(circuit)')
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:attr}Program information extracted by \CodeIn{QP\_Attribute}.}
\end{figure}

\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}
    '\textbf{Aer.get_backend}("qasm_simulator")'
    '\textbf{QuantumRegister}(3)'
    '\textbf{ClassicalRegister}(3)' 
    '\textbf{QuantumCircuit}(qreg,creg)'
    'circuit.\textbf{h}(0)'
    'circuit.\textbf{h}(2)'
    'circuit.\textbf{cx}(0,1)'
    'circuit.\textbf{measure}([0,1,2],[0,1,2])'
    '\textbf{execute}(circuit,simulator,shots=1000)'
    'job.\textbf{result}()'
    'result.\textbf{get_counts}(circuit)'
    '\textbf{print}(counts)'
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:opt}Program information extracted by \CodeIn{QP\_Operation}.}
\end{figure}


\subsection{Bug Pattern Detectors}

Bug patterns are erroneous code idioms or bad coding practices that have been proven to fail time and time again, which are usually caused by the misunderstanding of a programming language’s features, the use of erroneous design patterns, or simple mistakes sharing common behaviors. Previous work has identified some bug patterns for the Qiskit programming language~\cite{zhao2021identifying,zhao2021bugs4q}. In this work, we refined these bug patterns and built eight detectors to detect them. Table~\ref{table:1} shows the name of detectors and descriptions of bug patterns. We briefly describe each detector as follows.
%and the bug patterns can be found.
%Detailed descriptions and functions of each detector are explained as follows:
\begin{table}[h]
%\begin{CodeOutFN}
\caption{\label{table:1} Bug patterns that each detector is responsible for.}
\footnotesize{
\begin{center}
\renewcommand\arraystretch{1.5}
\begin{tabular} {c|l}
\hline 

\rowcolor{lightgray}\textbf{Detector Name}&\textbf{Bug patterns Descriptions}\\

\hline
\multirow{3}{0em}{\textbf{IG}} 
& - Gates are not among the backend’s basis gates. \\
& - Handle custom multi-qubit gates.\\
& - Random gate is not defined. \\
%&Wrong uses of gates lead to incorrect reset \\

\hline
\multirow{1}{0em}{\textbf{MI}} 
& - Ignoring the effects of measurement. \\

\hline
\multirow{3}{0em}{\textbf{IS}} 
& - Number of qubits larger than the registers defined. \\
& - The insufficient number of qubits.\\
& - Insufficient length of classical registers. \\

\hline
\multirow{6}{0em}{\textbf{PE}} 
& - Instruction not in basis gates. \\
& - Incorrect parameters in gates.\\
& - Using classical bits for entanglement. \\
& - Same physical qubit used in one operation. \\
%& Parameter error during decontrol operation. \\
& - Not giving lists for coupling\_map. \\

\hline 
\multirow{4}{0em}{\textbf{CM}} 
& - \zpz{Unrecognized parameters.} \\
& - Quantum circuit interaction error.\\
& - Create redundant classical registers. \\
& - The wrong command was used. \\

\hline 
\multirow{4}{0em}{\textbf{CE}} 
& - Object call error. \\
& - Import error.\\
& - Backend error. \\
& - Translating error. \\

\hline 
\multirow{1}{0em}{\textbf{QE}} 
& - Issue with new from\_qasm\_str() method. \\
\hline

\multirow{1}{0em}{\textbf{DO}} 
& - Method has been deprecated. \\

\hline

\end{tabular}
\end{center}
}
%\end{CodeOutFN}

\end{table}


\iffalse
\begin{table}[h]
%\begin{CodeOutFN}
\caption{\label{table:1} Bug patterns that each detector is responsible for.}
\footnotesize{
\begin{center}
\renewcommand\arraystretch{1.5}
\begin{tabular} {c|l}
\hline 

\rowcolor{lightgray}\textbf{Detector Code}&\textbf{Cases can be found}\\

\hline
\multirow{4}{0em}{\textbf{IG}} 
&Gates are not among the backend’s basis gates. \\
&Handle custom multi-qubit gates.\\
&Random gate is not defined. \\
%&Wrong uses of gates lead to incorrect reset \\

\hline
\multirow{1}{0em}{\textbf{IM}} 
&Ignoring the effects of measurement. \\

\hline
\multirow{3}{0em}{\textbf{IS}} 
&Number of qubits higher than the registers defined. \\
&The Insufficient number of qubits.\\
&Insufficient length of classical registers. \\

\hline
\multirow{6}{0em}{\textbf{PE}} 
& Instruction not in basis gates. \\
& Incorrect qubit parameters in gates.\\
& Using classical bits for entanglement. \\
& Same physical qubit used in one operation. \\
%& Parameter error during decontrol operation. \\
& Not giving lists for coupling\_map. \\

\hline 
\multirow{4}{0em}{\textbf{CM}} 
& Command misuse leads to unrecognized parameters. \\
& Quantum circuit mis-nesting.\\
& Create redundant classical registers. \\
& The Wrong command was used. \\

\hline 
\multirow{4}{0em}{\textbf{CE}} 
& Object call error. \\
& Import error.\\
& Backends error. \\
& Translate error. \\

\hline 
\multirow{1}{0em}{\textbf{QE}} 
& Issue with new from\_qasm\_str() method. \\
\hline

\multirow{1}{0em}{\textbf{DO}} 
& Method has been deprecated. \\

\hline

\end{tabular}
\end{center}
}
%\end{CodeOutFN}

\end{table}
\fi




\subsubsection{Incorrect uses of quantum gates (IG)}
This detector mainly checks if quantum gates are called correctly.
It determines whether a gate is recognized by Qiskit and whether it has been defined. In addition, the compliance of a custom gate and a three-qubit gate with the specification would also be checked.

\subsubsection{Measurement related issue (MI)}
Incorrect measurement means not only the improper use of measure operation that cause bugs but also the wrong operation after measurement. As shown in Figure~\ref{fig:5}, the user wants to achieve a quantum teleportation program.
The measured qubits are used as control qubits to entangle with other qubits.
\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}
    qc = \textbf{QuantumCircuit}(3, 3)
    qc.\textbf{x}(0)
    qc.\textbf{h}(1)
    qc.\textbf{cx}(1, 2)
    qc.\textbf{cx}(0, 1)
    qc.\textbf{h}(0)
    qc.\textbf{measure}(0, 0)
    qc.\textbf{measure}(1, 1)
    qc.\textbf{cx}(1, 2)       \textit{<- Problematic operation} 
    qc.\textbf{cz}(0, 2)       \textit{<- Problematic operation}
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:5}Example of Incorrect Mearsurement}
\end{figure}
This detector mainly acts after the \CodeIn{measure} method is called.
It iterates through the operations following the \CodeIn{measure} statement and determines whether the measured qubit appears as a control qubit in the double-qubit gate operations.

\subsubsection{Incorrect initial state (IS)} 
This checker does not simply check whether the definitions of \CodeIn{QuantumRegister} and \CodeIn{ClassicalRegister} conform to the specification. It determines whether the initialization satisfies the entire quantum program's operation on qubits.
Sometimes, the Qiskit program limits the number of qubits used when simulating quantum programs. Such as, after our validation, using \CodeIn{Aer.get\_backend('qasm\_simulator')} as backends supports less than 30 qubits for measure operation, while \CodeIn{BasicAer.get\_backend('qasm\_simulator')} supports less than 24 qubits.
In this case, the detector first checks the backend chosen by users and Identifies if the initialized qubits are out of limits.
When the number of initialized qubits is set to \CodeIn{n}, the checker will keep track of the number of qubits called in the program.



\subsubsection{Parameter error (PE)}
After a quantum gate is invoked, the detector is responsible for determining whether the parameters in the gate are correct, including the parameters that do not exist in multiple-qubit gates, and the wrong use of numeric types.
However, some bug patterns are not easy to find. From Figure~\ref{fig:6}, we can see that the user wants to assign the qubits in the register to the physical qubits, both \CodeIn{qreg[0]} are \CodeIn{qreg[5]} assigned to the physical qubits \CodeIn{12}. Therefore, the detector goes through the parameter values and checks for duplicate physical qubit occupancy.

\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}      
qreg = qk.\textbf{QuantumRegister}(7)

\textbf{layout} = \{qreg[0]: 12,     \textit{<- Problematic operation}
          qreg[1]: 11,
          qreg[2]: 13, 
          qreg[3]: 17, 
          qreg[4]: 14, 
          qreg[5]: 12,     \textit{<- Problematic operation}
          qreg[6]: 6\}
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:6}Example of parameters error}
\end{figure}



\subsubsection{Command misuse (CM)} 
This detector could detect the wrong or improper use of commands. Sometimes, parameters are not recognized because the method name is miswritten.
On the other hand, some methods can not recognize parameters and raise errors. As shown in Figure~\ref{fig:7}, attribute \CodeIn{pulse.shiftphase()} is not in module \CodeIn{qiskit.phase}.
Some of the commands in Qiskit are difficult to detect. For example, there are more than two quantum circuits while the user wants to nest one circuit with the others: 1) Command \CodeIn{to\_gate()} could be used to change the circuit into a combination of gates embedded in other circuits. 
2) Command \CodeIn{decompose()} could be used to decompose the circuit for embedded operation automatically.

%can not be recognized by the circuit library.
%If the detector finds the unrecognized parameter, it will traverse the entire program to find the \CodeIn{decompose()}, which is needed by the circuit library.

\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}      
phase = \textbf{Parameter}('phase')

\textbf{with} pulse.build(FakeAlmaden())\textbf{as} phase_test_sched:

        pulse.\textbf{shiftphase}(            \textit{<- Unrecognized}
        phase, pulse.\textbf{drive_channel}(0))

phase_test_sched.\textbf{instructions}
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:7}Example of command misuse.}
\end{figure}

\iffalse
\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}      
ansatz = \textbf{RealAmplitudes}(num_qubits=1, reps=1)

for method in ['param_shift',
                'fin_diff', 
                'lin_comb']:
                
    grad = \textbf{Gradient}(method).       \textbf{<-} Unrecognized
           convert(CircuitStateFn(ansatz))
           
    \textbf{print}(f"{method} is ok")
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:7}Example of command misuse.}
\end{figure}
\fi

\subsubsection{Call error (CE)} 
This checker is responsible for call errors, including Python package calls, backend simulator calls, and translator calls.
Besides, the detector can check for problems with parameter declarations. As shown in Figure~\ref{fig:8}, this error is not a duplicate call to \CodeIn{PauliMeasurementBasis()}. After running the code, we found that there was an error of \textit{invalid qubits for basis}. The call of \CodeIn{PauliMeasurementBasis()} is invalid for \CodeIn{preparation\_basis}.
This kind of bug is hard to detect by QChecker, the detector can only judge one scenario now. 
\begin{figure}[t]
  \begin{CodeOut}
\footnotesize{
  \begin{alltt}      
circ = QuantumCircuit(1,1)
circ.x(0)

tomo = ProcessTomography(
       circuit=circ,
       measurement_basis=PauliMeasurementBasis(),
       measurement_qubits=None,
       preparation_basis=PauliMeasurementBasis(),\textit{ <-}
       preparation_qubits=None,
       basis_indices=None,
       qubits=None)
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:8}Example of call error}
\end{figure}

\subsubsection{QASM error (QE)} 
This checker detects problems with \CodeIn{qasm\_simulator} as the backend or when building \textit{qasm} programs with the Qiskit programming language.

\subsubsection{Discarded orders (DO)}
This detector determines if a deprecated method is being called, and it comes into play when an old operation or variable type is discarded due to a version update.





\iffalse
\begin{itemize}[leftmargin=2em]
\setlength{\itemsep}{3pt}
\item \textbf{Incorrect uses of quantum gates (IG)}. This detector mainly checks if quantum gates are called correctly.
It determines whether a gate is recognized by Qiskit and whether it has been defined. {\color{red}In addition, the compliance of a custom gate and a three-qubit gate with the specification could also be checked.}
  
\item \textbf{Measurement related issue (MI)}. This detector mainly acts after the \CodeIn{measure} method is called.
It detects whether a measured qubit creates entanglement with other qubits.
  
\item \textbf{Parameters error (PE)}. After a quantum gate is invoked, the detector is responsible for determining whether the parameters in the gate are correct and whether the qubits come from the classical register.
  
\item \textbf{Incorrect initial state (IS)}. This checker does not simply check whether the definitions of \CodeIn{QuantumRegister} and \CodeIn{ClassicalRegister} conform to the specification. It determines whether the initialization satisfies the entire quantum program's operation on qubits.

\item \textbf{Command misuse (CM)}. This checker could detect the wrong or improper use of commands. Sometimes, parameters are not recognized because the method name is miswritten.
\item \textbf{Call error (CE)}. This checker is responsible for call errors, including Python package calls, backend simulator calls, and translator calls. 
\item \textbf{QASM error (QE)}. This checker detects problems with \CodeIn{qasm\_simulator} as the backend or when building \textit{qasm} programs with the Qiskit programming language.
\end{itemize}
\fi

\subsection{Bug Detection}
The bug patterns shown in Table~\ref{table:1} represent the general bugs in quantum programs. In addition to syntactic bugs, it also contains some faulty logic in some quantum-related operations.
Based on the program information extraction modules (\CodeIn{QP\_Attribute}
and \CodeIn{QP\_Operation}),
as well as the detectors (e.g., IG, MI, etc.), 
we can perform a thorough static test for the quantum program files. To enable comprehensive and useful bug detection and benefit the debug process, we report the details of the buggy programs (code lines, content, etc.), bug types (patterns), and specific descriptions. We hope such information helps users improve the quality of quantum programs.












==> sections/related-work.tex <==
\section{Related work}\label{sec:related}
% This section briefly discusses the following lines of closely related research.

\subsection{Static Analysis Techniques for Traditional Software}
The application of static analysis tools for traditional software defect detection is a common practice for developers and has been extensively studied by previous researchers~\cite{flanagan2002extended, nagappan2005static, nanda2010making, vassallo2020developers, iberia2022tor}. 
The bug patterns proposed in~\cite{hovemeyer2004finding} is an efficient technique for finding bugs in real-world software. \textit{Formal Proof}~\cite{cook2006termination} is an effective static technique for eliminating bugs. Though the existence of correctness proof is the best guarantee that the program does not contain bugs, constructing such proof is still prohibitive for most programs. \textit{Partial verification}~\cite{henzinger2002lazy} techniques have been proposed to prove that some desired program properties hold for all possible executions.
In addition, several static analysis tools exist for Python programs~\cite{thenault2001pylint, liu2019static, pyflakes}, which have achieved excellent outcomes in detecting defects in Python programs. However, the existing static analysis tools struggle to detect quantum-related bugs in quantum programs. Since the quantum computation logic is expressed in quantum circuits, the states of quantum registers are measured probabilistically. QChecker proposes a novel approach consisting of a decomposition of quantum programs and a set of refined bug patterns that enables it to perform static analysis on quantum programs.
%, unlike previous work.

\subsection{Testing Techniques for Quantum Computing}
%\subsubsection{Testing and manipulating quantum programs}
\textcolor{cyan}{
Several testing tools and test case generation methods for quantum programs have been proposed.
Quito~\citep{wang2021quito} provides three coverage criteria for quantum programs and their test generation strategies. QuCAT~\citep{gely2020qucat} provides two schemes for generating combinatorial test suites.
%and argues that the more intense combinatorial tests are superior in effectiveness to the less intense ones. 
QuSBT~\citep{wang2021generating} is a search-based testing method,
that aims to maximize the number of failed test cases in the test suite.
%that designs 30 buggy versions for six quantum programs to demonstrate their effectiveness. 
%These studies have contributed to the advancement of quantum program testing.
%Although we would like to be able to verify the effectiveness of these methods and tools on Bug4Q, unfortunately, these tools are not available for application to Bugs4Q. 
Muskit~\citep{mendiluze2021muskit} is a quantum mutation analysis tool for the Qiskit language, focusing on mutation operators for quantum gates. QMutPy~\citep{fortunato2022mutation,fortunato2022mutation2} can generate effective mutation programs for \textit{measurement} calls and a large number of quantum gates. 
%The above mutation tools can effectively generate various mutation program instances to enrich the testing.
}
\zpz{
Besides, Huang and Martonosi~\cite{huang2018qdb,huang2019statistical} proposed a statistical assertion strategy to find bugs and offered a defense strategy for writing defect-free code.
QDiff~\cite{wang2022qdiff} proposed differential testing and achieved its acceleration by analyzing the static characteristics of quantum circuits.
Different from previous works, QChecker is a static analysis tool for quantum programs.
}

%\textcolor{red}{To the best of our knowledge, QChecker is the first static analysis tool for quantum programs.}

%\textcolor{red}{Zhao: (1) to refine the related work on the above quantum software testing, (2) to add some related work on program analysis of quantum programs, especially those for bug findings}

\iffalse
\subsubsection{Quantum computing platforms} A study by~\cite{zhao2021bugs4q} collects a dataset of 42 real-world bugs in Qiskit and Cirq and identifies crashes and wrong outputs as the most common impact of quantum bugs, which inspires this work. We refine the bug patterns proposed in this study to build QChecker. Wang \emph{et al.}~\cite{wang2022qdiff} propose QDiff, the first differential testing technique for quantum computing frameworks. QDiff starts from a small set of manually written programs and generates variants based on these hand-written programs to perform differential testing across different backends and optimization levels of quantum computing frameworks. Paltenghi and Pradel~\cite{matteo2022morphq} propose MorphQ, the first metamorphic testing approach for a quantum computing framework. MorphQ consists of a program generator to create a large and diverse set of valid quantum programs and a set of program transformations that can exploit the quantum-specific metamorphic relationship, which enables MorphQ to perform metamorphic testing on Qiskit. While QDiff and MorphQ focus on testing quantum computing frameworks, QChecker mainly performs static analysis on quantum programs.
\fi

==> sections/threats.tex <==
\section{Treats to Validity}\label{sec:threats}

%\subsection{External Threats}
The number of bug patterns can be a threat to validity. We have put much effort into collecting bugs from quantum programs and extracting as many bug patterns as possible from these collected bugs. However, due to the limitation of the current scale of development and application of quantum programs, we cannot include more bug patterns in QChecker. Therefore, we will continue to collect quantum programs and their bugs, enrich QChecker's detection capabilities, and continuously update the tool. Nevertheless, the evaluation of Bugs4Q shows that QChecker can still detect bugs in various quantum programs.

% The number of bug patterns can be a threat of validity.
% We have invested efforts to limited by the number of bugs in the quantum program, we .
% In addition, QChecker has not been evaluated extremely well. 
% Limited by the size of the quantum program, it may not take much time and resources to execute the quantum program, which does not reflect the value of QChecker.
% When large-scale quantum programs are available, QChecker can be well-evaluated.

%\subsection{Internal Threats}
%QChecker supports detecting Python-based quantum programming languages (e.g., Qiskit, Cirq, ProjectQ). 
QChecker is designed for Qiskit, and it can be extended to other Python-based quantum languages (e.g., Cirq) with slight modification.
However, it also has limitations. For instance, ProjectQ has overloaded the \begin{math}|\end{math} operator, which will cause the information extractor fails to work. As shown in Figures~\ref{fig:12} and \ref{fig:13}, QChecker could not extract information from the underlying ProjectQ program, such as the \CodeIn{H} gate and \CodeIn{CX} gate. These limitations will be resolved with the extension of QChecker.
%which leads to the detectors failing to work. 
%In addition, some of the detectors in QChecker could only cover a limited number of cases. 
%And the detectors can only provide error codes while not locating specific error statements.
%In future work, we plan to integrate QChecker into Microsoft Visual Studio Code~\cite{code2019visual} as an extension and provide the corresponding features.
%Finally, QChecker does not support detecting quantum programming languages which are not Python-based, such as Q\#. We leave these issues as future works for QChecker.


\begin{figure}[t]
\begin{CodeOut}
    \footnotesize{
  \begin{alltt}
    eng = \textbf{MainEngine}()
    qubits = eng.allocate_qureg(3)
    \textbf{H} | qubits[0]
    \textbf{CX} | (qubits[0], qubits[2])
    eng.flush()
    amplitudes = np.array(eng.backend.cheat()[1])
    amplitudes = np.abs(amplitudes)
    \textbf{All(Measure)} | qubits
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:12}An exapmle of ProjectQ program.}
\end{figure}

\begin{figure}[t]
\begin{CodeOut}
    \footnotesize{
  \begin{alltt}
    ('eng', '\textbf{MainEngine}()')
    ('qubits', 'eng.allocate_qureg(3)')
    ('amplitudes', 'np.array([1])')
    ('amplitudes', 'np.abs(amplitudes)')
    ==========================================
    '\textbf{MainEngine}()'
    'eng.allocate_qureg(3)'
    'eng.flush()'
    'np.array([1])'
    'np.abs(amplitudes)'
    '\textbf{All(Measure)}'
    'eng.backend.cheat()']
  \end{alltt}
}
\end{CodeOut}
\Caption{\label{fig:13}A ProjectQ program detected by QChecker.}
\end{figure}

\textcolor{red}{
%\subsection{Verifiability}
%This threat concerns the possibility of replicating this research.
Considering the verifiability of this work,
we provide all the necessary details to help researchers replicate this work. The replication package is made publicly available at \url{https://github.com/Z-928/QChecker}.
} 
